Feature Re-Learning with Data Augmentation for Video Relevance Prediction

Predicting the relevance between two given videos with respect to their visual content is a key component for content-based video recommendation and retrieval. Thanks to the increasing availability of pre-trained image and video convolutional neural network models, deep visual features are widely used for video content representation. However, as how two videos are relevant is task-dependent, such off-the-shelf features are not always optimal for all tasks. Moreover, due to varied concerns including copyright, privacy and security, one might have access to only pre-computed video features rather than original videos. We propose in this paper feature re-learning for improving video relevance prediction, with no need of revisiting the original video content. In particular, re-learning is realized by projecting a given deep feature into a new space by an affine transformation. We optimize the re-learning process by a novel negative-enhanced triplet ranking loss. In order to generate more training data, we propose a new data augmentation strategy which works directly on frame-level and video-level features. Extensive experiments in the context of the Hulu Content-based Video Relevance Prediction Challenge 2018 justify the effectiveness of the proposed method and its state-of-the-art performance for content-based video relevance prediction.

==> table-testset.tex <==
\begin{table*} [tb!]
\renewcommand{\arraystretch}{1.2}
\caption{Performance comparison on the test set. Our runs outperform the Hulu's best baseline with a large margin. The number in the bracket indicates the relative improvement over the Hulu baseline. }
\label{tab:perf-on-test}
\centering
 \scalebox{0.8}{
     \begin{tabular}{@{} l*{9}{c} l*{9}{c} @{}}
\toprule
         & \multicolumn{9}{c}{\textbf{Track 1: TV-shows}} & \multicolumn{9}{c}{\textbf{Track 2: Movies}} \\
         \cmidrule(r){2-10} \cmidrule(r){12-20}
         \multirow{2}{*}{} & \multicolumn{4}{c}{\textbf{hit@k}} &  & \multicolumn{4}{c}{\textbf{recall@k}} & \multicolumn{4}{c}{\textbf{hit@k}} &  & \multicolumn{4}{c}{\textbf{recall@k}} \\
         \cmidrule(r){2-5}  \cmidrule(r){7-10} \cmidrule(r){12-15}  \cmidrule(r){17-20}
         & k=5 & k=10 & k=20 & k=30 & &  k=50 & \blue{k=100} & k=200 & k=300 & &  k=5 & k=10 & k=20 & k=30 & &  k=50 & \blue{k=100} & k=200 & k=300 \\
\midrule
% \cmidrule(r){1-10} \cmidrule(r){12-20}
%\hline
         \textbf{Hulu}       & 0.249 & 0.356 & 0.461 & 0.525     &  &  0.085 & \blue{0.141}  & 0.219 & 0.269 
                           && 0.190 & 0.242 & 0.320 & 0.373     &  &  0.081 & \blue{0.116} & 0.168 & 0.206 \\ [1pt]
% \midrule
         \textbf{run 1}       & 0.274 & 0.365 & 0.488 & 0.542     &  &  0.099 & \blue{0.160} ($\uparrow$ 13.5\%) & 0.248 & 0.302 
                            && 0.210 & 0.272 & 0.355 & 0.412     &  &  0.092 & \blue{0.133} ($\uparrow$ 14.7\%)& 0.192 & 0.237 \\
         \textbf{run 2}       & 0.287 & 0.381 & 0.492 & 0.550     &  &  0.104 & \blue{0.167} ($\uparrow$ 18.4\%)& 0.257 & 0.314
                            && 0.211 & 0.278 & 0.368 & 0.427     &  &  0.095 & \blue{0.139} ($\uparrow$ 19.8\%)& 0.201 & 0.248 \\
         \textbf{run 3}       & 0.288 & 0.391 & 0.484 & 0.539     &  &  0.099 & \blue{0.162} ($\uparrow$ 14.9\%)& 0.249 & 0.305
                            && 0.215 & 0.278 & 0.359 & 0.422     &  &  0.096 & \blue{0.138} ($\uparrow$ 19.0\%)& 0.198 & 0.244 \\
         \textbf{run 4}       & \textbf{0.309} & \textbf{0.411} & 0.506 & 0.567     &  &  0.109 & \blue{0.173} ($\uparrow$ 22.7\%)& 0.266 & 0.323 
                            && \textbf{0.234} & 0.298 & \textbf{0.390} & \textbf{0.448}     &  &  0.104 &  \blue{0.148} ($\uparrow$ 27.6\%)& 0.210 & 0.258 \\
         \textbf{run 5}       & 0.308 & 0.408 & \textbf{0.522} & \textbf{0.589}     &  &  \textbf{0.112} & \blue{\textbf{0.178}} ($\uparrow$ 26.2\%)& \textbf{0.273} & \textbf{0.331}
                            && 0.232 & \textbf{0.302} & 0.389 & 0.441     &  &  \textbf{0.105} & \blue{\textbf{0.151}} ($\uparrow$ 30.2\%)& \textbf{0.215} & \textbf{0.263} \\
\bottomrule
\end{tabular}
 }% end of scalebox
\end{table*}

